Attributed Graph Modeling with Vertex Replacement Grammars

Recent work at the intersection of formal language theory and graph theory has explored graph grammars for graph modeling. However, existing models and formalisms can only operate on homogeneous (i.e., untyped or unattributed) graphs. We relax this restriction and introduce the Attributed Vertex Replacement Grammar (AVRG), which can be efficiently extracted from heterogeneous (i.e., typed, colored, or attributed) graphs. Unlike current state-of-the-art methods, which train enormous models over complicated deep neural architectures, the AVRG model is unsupervised and interpretable. It is based on context-free string grammars and works by encoding graph rewriting rules into a graph grammar containing graphlets and instructions on how they fit together. We show that the AVRG can encode succinct models of input graphs yet faithfully preserve their structure and assortativity properties. Experiments on large real-world datasets show that graphs generated from the AVRG model exhibit substructures and attribute configurations that match those found in the input networks.

==> data/link-pred-table.tex <==
\begin{tabular}{llrrrrrr}
\toprule
          &            & \multicolumn{3}{l}{mean} & \multicolumn{3}{l}{std} \\
          &            &     AP &   AUPR &  AUROC &     AP &   AUPR &  AUROC \\
name & model &        &        &        &        &        &        \\
\midrule
citeseer & AVRG &  0.628 &  0.811 &  0.628 &  0.005 &  0.006 &  0.005 \\
          & adamic-adar &  0.766 &  0.879 &  0.765 &  0.007 &  0.003 &  0.007 \\
          & gcn\_ae &  0.934 &  0.933 &  0.910 &  0.008 &  0.008 &  0.010 \\
          & gcn\_vae &  0.931 &  0.931 &  0.909 &  0.007 &  0.007 &  0.010 \\
          & jaccard &  0.759 &  0.873 &  0.764 &  0.009 &  0.008 &  0.007 \\
          & linear\_ae &  0.928 &  0.928 &  0.900 &  0.008 &  0.008 &  0.013 \\
          & linear\_vae &  0.939 &  0.939 &  0.919 &  0.006 &  0.006 &  0.010 \\
cora & AVRG &  0.601 &  0.796 &  0.602 &  0.008 &  0.006 &  0.009 \\
          & adamic-adar &  0.758 &  0.873 &  0.758 &  0.014 &  0.011 &  0.013 \\
          & gcn\_ae &  0.913 &  0.913 &  0.887 &  0.010 &  0.010 &  0.015 \\
          & gcn\_vae &  0.914 &  0.914 &  0.891 &  0.006 &  0.006 &  0.007 \\
          & jaccard &  0.752 &  0.866 &  0.757 &  0.016 &  0.012 &  0.014 \\
          & linear\_ae &  0.904 &  0.904 &  0.871 &  0.010 &  0.010 &  0.012 \\
          & linear\_vae &  0.919 &  0.919 &  0.895 &  0.006 &  0.006 &  0.006 \\
cornell & AVRG &  0.608 &  0.779 &  0.606 &  0.047 &  0.055 &  0.048 \\
          & adamic-adar &  0.741 &  0.788 &  0.700 &  0.053 &  0.053 &  0.062 \\
          & gcn\_ae &  0.781 &  0.778 &  0.684 &  0.049 &  0.050 &  0.070 \\
          & gcn\_vae &  0.797 &  0.794 &  0.704 &  0.058 &  0.059 &  0.091 \\
          & jaccard &  0.541 &  0.570 &  0.603 &  0.044 &  0.063 &  0.062 \\
          & linear\_ae &  0.764 &  0.759 &  0.673 &  0.056 &  0.058 &  0.077 \\
          & linear\_vae &  0.809 &  0.805 &  0.734 &  0.048 &  0.049 &  0.058 \\
texas & AVRG &  0.608 &  0.786 &  0.609 &  0.028 &  0.050 &  0.032 \\
          & adamic-adar &  0.713 &  0.770 &  0.686 &  0.024 &  0.029 &  0.047 \\
          & gcn\_ae &  0.619 &  0.611 &  0.487 &  0.062 &  0.064 &  0.079 \\
          & gcn\_vae &  0.660 &  0.654 &  0.533 &  0.059 &  0.060 &  0.079 \\
          & jaccard &  0.529 &  0.548 &  0.578 &  0.075 &  0.090 &  0.090 \\
          & linear\_ae &  0.616 &  0.609 &  0.472 &  0.047 &  0.048 &  0.065 \\
          & linear\_vae &  0.721 &  0.715 &  0.630 &  0.062 &  0.064 &  0.083 \\
wisconsin & AVRG &  0.610 &  0.794 &  0.612 &  0.029 &  0.021 &  0.030 \\
          & adamic-adar &  0.689 &  0.751 &  0.660 &  0.037 &  0.049 &  0.051 \\
          & gcn\_ae &  0.762 &  0.760 &  0.660 &  0.037 &  0.038 &  0.059 \\
          & gcn\_vae &  0.779 &  0.776 &  0.693 &  0.038 &  0.038 &  0.055 \\
          & jaccard &  0.564 &  0.612 &  0.610 &  0.058 &  0.079 &  0.057 \\
          & linear\_ae &  0.765 &  0.763 &  0.662 &  0.043 &  0.043 &  0.067 \\
          & linear\_vae &  0.790 &  0.788 &  0.715 &  0.051 &  0.051 &  0.068 \\
\bottomrule
\end{tabular}



==> figs/results-table.tex <==
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}
\toprule
{}     & \multicolumn{3}{c}{Polbooks}                     & \multicolumn{3}{c}{Football}                     & \multicolumn{3}{c}{Texas}                        & \multicolumn{3}{c}{Cornell}                      \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(ll){11-13}  
{}     & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             \\ \midrule
AGM    & \textbf{0.058} & 0.062          & 0.087          & --             & --             & --             & --             & --             & --             & --             & --             & --             \\ 
AVRG   & 0.171          & 0.080          & 0.229          & \textbf{0.022} & \textbf{0.056} & \textbf{0.051} & \textbf{0.030} & \textbf{0.036} & \textbf{0.118} & 0.042          & 0.031          & \textbf{0.081} \\
CELL   & \ul{0.069}    & 0.164          & \textbf{0.058} & \ul{0.103}    & \ul{0.086}    & \ul{0.125}    & \ul{0.048}    & \ul{0.038}    & \ul{0.132}    & \textbf{0.032} & \textbf{0.021} & \ul{0.085}    \\
CL     & 0.729          & 0.075          & \ul{0.069}    & 0.618          & 0.176          & 0.178          & 0.276          & 0.097          & 0.265          & 0.058          & 0.091          & 0.226          \\
DC-SBM & 0.115          & \ul{0.037}    & 0.194          & 0.197          & 0.142          & 0.254          & 0.253          & 0.051          & 0.221          & 0.052          & 0.056          & 0.208          \\
NetGAN & 0.112          & \textbf{0.030} & 0.192          & 0.170          & 0.159          & 0.189          & 0.173          & 0.049          & 0.203          & \ul{0.037}    & \ul{0.023}    & 0.153          \\
GAE    & 0.280          & 0.093          & 3.014          & 0.444          & 0.208          & 2.430          & 0.326          & 0.592          & 5.584          & 0.062          & 0.671          & 5.916          \\
GVAE   & 0.259          & 0.081          & 3.826          & 0.503          & 0.199          & 3.454          & 0.302          & 0.754          & 6.433          & 0.093          & 0.754          & 6.235          \\
\\ 
%
%
{}     & \multicolumn{3}{c}{Wisconsin}                    & \multicolumn{3}{c}{Airports}                     & \multicolumn{3}{c}{Polblogs}                     & \multicolumn{3}{c}{Citeseer}                     \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(ll){11-13} 
{}     & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             \\ \midrule
AGM    & --             & --             & --             & 0.048          & 0.211          & \ul{0.185}    & \textbf{0.024} & 0.142          & 0.224          & \textbf{0.012} & \textbf{0.021} & 0.022          \\ 
AVRG   & \textbf{0.020} & \textbf{0.025} & \ul{0.136}    & \ul{0.063}    & 0.041          & 0.447          & 0.283          & 0.083          & 0.357          & 0.263          & 0.034          & \ul{0.018}    \\
CELL   & \ul{0.029}    & \textbf{0.025} & \textbf{0.111} & \textbf{0.038} & \textbf{0.011} & 0.194          & \ul{0.028}    & \ul{0.026}    & \textbf{0.107} & \ul{0.200}    & 0.058          & 0.024          \\
CL     & 0.147          & 0.070          & 0.195          & 0.359          & 0.226          & \textbf{0.154} & 0.814          & 0.159          & \ul{0.150}    & 0.669          & 0.026          & \textbf{0.015} \\
DC-SBM & 0.139          & 0.035          & 0.150          & 0.048          & \ul{0.025}    & 0.523          & 0.032          & \textbf{0.023} & 0.291          & 0.314          & \ul{0.022}    & \ul{0.018}    \\
NetGAN & 0.115          & 0.035          & 0.198          & 0.152          & 0.148          & 0.589          & 0.367          & 0.154          & 0.323          & 0.602          & 0.051          & 0.032          \\
GAE    & 0.182          & 0.451          & 6.595          & 0.154          & 0.029          & 13.518         & 0.218          & 0.167          & 16.025         & 0.612          & 0.027          & 20.260         \\
GVAE   & 0.190          & 0.547          & 7.216          & 0.183          & 0.226          & 13.685         & 0.222          & 0.142          & 16.079         & 0.609          & 0.059          & 20.764         \\
\\
%
%
{}     & \multicolumn{3}{c}{Chameleon}                    & \multicolumn{3}{c}{Cora}                         & \multicolumn{3}{c}{Squirrel}                     & \multicolumn{3}{c}{Film}                         \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(ll){11-13} 
{}     & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             & $\Delta \rho_{\text{attr}}$           & $\Delta \rho_{\text{deg}}$            & $\lambda$-dist             \\ \midrule
AGM    & 0.036          & 0.125          & 0.196          & \textbf{0.013} & 0.032          & 0.026          & 0.008          & 0.083          & 0.521          & \ul{0.004}    & 0.020          & 0.047          \\
AVRG   & \textbf{0.007} & \ul{0.010}    & \textbf{0.072} & 0.374          & 0.042          & 0.026          & 0.006          & 0.067          & \ul{0.356}    & \textbf{0.003} & \ul{0.006}    & \ul{0.025}    \\ 
CELL   & 0.017          & \textbf{0.003} & 0.260          & \ul{0.132}    & \textbf{0.004} & \ul{0.022}    & \textbf{0.001} & \textbf{0.030} & \textbf{0.303} & \ul{0.004}    & \textbf{0.001} & \textbf{0.023} \\
CL     & 0.035          & 0.129          & \ul{0.174}    & 0.766          & 0.046          & \textbf{0.015} & 0.007          & 0.095          & 0.472          & \textbf{0.003} & 0.019          & 0.039          \\
DC-SBM & \ul{0.012}    & 0.017          & 0.361          & 0.292          & \ul{0.020}    & 0.024          & \ul{0.002}    & \ul{0.034}    & 0.835          & \ul{0.004}    & 0.008          & 0.030          \\
NetGAN & 0.029          & 0.129          & 0.332          & 0.710          & 0.036          & 0.058          & 0.008          & 0.219          & 1.041          & --             & --             & --             \\
GAE    & --             & --             & --             & 0.688          & 0.066          & 22.364         & --             & --             & --             & --             & --             & --             \\
GVAE   & --             & --             & --             & 0.686          & 0.058          & 21.860         & --             & --             & --             & --             & --             & --  \\
\bottomrule
\end{tabular}

==> plots/first-results-table.tex <==
\input{data/first-results}

\pgfplotstabletypeset[
    col sep=space,
    columns={name,model,ld},
    columns/name/.style={string type},
    columns/model/.style={string type},
    ]{
    name    model    ld  ld95    deg deg95   attr    attr95
airports AVRG 0.4467 0.007 0.041 0.0061 0.063 0.0068
chameleon AVRG 0.0723 0.0013 0.0098 0.0013 0.0068 0.0015
citeseer AVRG 0.0179 0.0015 0.0339 0.0073 0.2633 0.005
cora AVRG 0.0263 0.0015 0.0423 0.004 0.3745 0.0075
cornell AVRG 0.0811 0.0157 0.0313 0.0183 0.0418 0.0298
film AVRG 0.0248 0.0009 0.0061 0.0008 0.0031 0.0017
football AVRG 0.0512 0.0083 0.0561 0.0284 0.0224 0.0084
polblogs AVRG 0.3569 0.0049 0.0829 0.0062 0.2834 0.0233
polbooks AVRG 0.2289 0.0218 0.0796 0.0334 0.1711 0.0533
squirrel AVRG 0.3564 0.0041 0.0672 0.0017 0.0057 0.0006
texas AVRG 0.1182 0.0124 0.0357 0.0119 0.0295 0.0106
wisconsin AVRG 0.1358 0.0231 0.025 0.0136 0.0197 0.0125
    }
